Inductive Program Synthesis Over Noisy Data

We present a new framework and associated synthesis algorithms for program synthesis over noisy data, i.e., data that may contain incorrect/corrupted input-output examples. This framework is based on an extension of finite tree automata called {\em weighted finite tree automata}. We show how to apply this framework to formulate and solve a variety of program synthesis problems over noisy data. Results from our implemented system running on problems from the SyGuS 2018 benchmark suite highlight its ability to successfully synthesize programs in the face of noisy data sets, including the ability to synthesize a correct program even when every input-output example in the data set is corrupted.

==> dsl.tex <==
%\section{Key Definitions}
%Within this section, we will introduce some key definitions
%used within this paper.

\section{Domain Specific Languages}
\label{sec:dsl}

We first define the programs we consider, how inputs to the program are 
specified, and the program semantics. Without loss of generality, we assume
programs are specified as a tree (parse tree), where 
leaves are constants/0-arity symbols in the DSL. Internal nodes represent function invocations. 
A program $p$ executes in an input environment $\sigma$ with $\llbracket p \rrbracket \sigma$ the
output of $p$ on input $\sigma$ ($\llbracket . \rrbracket$ is defined in Figure~\ref{fig:exec_sem}).

\begin{figure}
    \[
        \begin{array}{c}
            \begin{array}{cc}
            \infral{}
            {\llbracket c \rrbracket \sigma \Rightarrow c}
            {(Constant)}
            &
            \infral{}
            {\llbracket x \rrbracket \sigma \Rightarrow \sigma(x)}
            {(Variable)}
            \end{array}
            \\
            \\
            \infral{
            \llbracket n_1 \rrbracket \sigma \Rightarrow v_1 ~~~~~ 
            \llbracket n_2 \rrbracket \sigma \Rightarrow v_2 ~~~~ \ldots ~~~~
            \llbracket n_k \rrbracket \sigma \Rightarrow v_k
            }
            {\llbracket f(n_1, n_2, \ldots n_k) \rrbracket \sigma  \Rightarrow
            f(v_1, v_2, \ldots v_k)}{(Function)}
    \end{array}
    \]
    \caption{Execution semantics for program $p$}
    \label{fig:exec_sem}
\end{figure}

All valid programs (which can be executed) 
in our DSL are defined by a grammar $G = (T, N, P, s_0)$ where:
\begin{itemize}
    \item $T$ is a set of terminal symbols. These may include 
        constants and symbols which change value depending on the environment
        $\sigma$.
    \item $N$ is the set of non-terminals that represent sub-expression in our
        DSL.
    \item $P$ is the set of production rules of the form \\ $s \rightarrow f(s_1,
        \ldots, s_n)$ where $f$ is a built in function in our DSL and 
        $s, s_1, \ldots, s_n$ are non-terminals in our grammar.
    \item $s_0 \in N$ is the start non-terminal in the grammar.
\end{itemize}


We assume that we are given a black box implementation of each function $f$
in the DSL.  In general, all techniques explored within this paper can be generalized to
any DSL which can be specified within the above framework.

\begin{example}\label{ex:dsl}
    Consider the following simple toy DSL. This DSL contains two constants and
    allows for addition and multiplication by these constants:
    \[
        \begin{array}{rcl}
            n &:=& \mathsf{id}(x) \alt n + t \alt n \times t; \\
            t &:=& 2 \alt 3;
        \end{array}
    \]
    Here, $\mathsf{id}$ is the identity function.
\end{example}

\iffalse
We work the following DSL in this paper.

\iffalse
\subsection{Integer Manipulation}
Figure~\ref{fig:int_lang} defines a basic integer manipulation language. 
The language allows us to express programs which 
take an integer $x$ as an input, then manipulates $x$ using the $+, \times, -,
\mathsf{Min}$ and $\mathsf{Max}$ operators.

\begin{figure}
    \[
        \begin{array}{rcl}
            \text{Integer expr} ~~~~~ e &:=& id(x)~\vert~k~\vert~e_1 +
            e_2~\vert~e_1 \times e_2~\vert~-e\\
            &\vert& \mathsf{Max}(e_1, e_2)~\vert~\mathsf{Min}(e_1, e_2);\\
        \end{array}
    \]
    \caption{DSL for integer manipulation, $k$ is an integer}
    \label{fig:int_lang}
\end{figure}
\fi

\subsection{String Transformations}
Automatic string transformations have been extensively studied
within the Programming by Example community~\cite{gulwani2011automating, polozov2015flashmeta,
singh2016transforming}. We adopt the 
DSL presented by~\cite{wang2017program} as shown in Fig~\ref{fig:str_lang}. The DSL
allows us to concatenate substrings ($\mathsf{Concat}$) of input string $x$, where each substring
is extracted using the $\mathsf{SubStr}$ function using a start and an end
position. A position can either be a constant index ($\mathsf{ConstPos}$) or 
the start or end of the $k^{th}$ occurrence of the match token $\tau$ 
in the input string ($\mathsf{Pos}$).


\begin{figure}
    \[
        \begin{array}{rcl}
            \text{String expr} ~~~~ e &:=&
            \mathsf{Str}(f)~\vert~\mathsf{Concat}(f, e);\\
            \text{Substring expr} ~~~~ f &:=& \mathsf{ConstStr}(s)~\vert~
            \mathsf{SubStr}(x, p_1, p_2);\\
            \text{Position} ~~~~ p &:=& \mathsf{Pos}(x, \tau, k, d)~\vert~
            \mathsf{ConstPos}(k)\\ &\vert&\mathsf{AddPos}(p, k);\\
            \text{Direction} ~~~~ d &:=& \mathsf{Start}~\vert~\mathsf{End};\\
        \end{array}
    \]
    \caption{DSL for string transformation, $\tau$ is a token, $k$ is an
    integer, and $s$ is a string constant}
    \label{fig:str_lang}
\end{figure}
\fi

\iffalse
\subsection{Matrix and Tensor Transformations}
This DSL (Figure~\ref{fig:ten_lang}) is motivated by prior work on learning tensor manipulations 
using examples~\cite{wang2017program}. The DSL includes tensor operators
$\mathsf{Reshape}$
(given a tensor $t$ and a vector $v$, reshape $t$ so that its dimensions become
$v$)
, $\mathsf{Permute}$ (given a tensor $t$ and a vector $v$, 
rearrange the dimensions of tensor $t$ so they are in the order specified 
by vector $v$), $\mathsf{Fliplr}$ (given tensor $t$, flip its columns in the
left-right directions) and $\mathsf{Flipud}$ (given a tensor $t$, flip its
rows in the up-down direction). Refer to~\cite{wang2017program} 
(or the corresponding MATLAB definitions available at www.mathworks.com/help/matlab/ref/x.html, 
where x is the name of the corresponding function)
for a precise specification of this DSL.

\begin{figure}
    \[
        \begin{array}{rcl}
            \text{Tensor expr} ~~~~~ t &:=& \mathsf{id}(x)~\vert~\mathsf{Reshape}(t,
            v)\\
            &\vert& \mathsf{Permute}(t, v)
            ~\vert~\mathsf{Fliplr}(t)~\vert~\mathsf{Flipud}(t);\\
        \text{Vector expr} ~~~~~ v &:=& [k_1, k_2] ~\vert~\mathsf{Cons}(k, v);\\
        \end{array}
    \]
    \caption{DSL for matrix  transformations where $k$ is an integer}
    \label{fig:ten_lang}
\end{figure}


\fi


==> mixtable.tex <==
\begin{figure*}
\begin{center}
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|}
\hline
    \multirow{2}{*}{Benchmark-1} & \multirow{2}{*}{Benchmark-2} &
    \multirow{2}{*}{No. of Examples} & \multirow{2}{*}{Switch $b$}&
    \multirow{2}{*}{One of the original Programs}& 
    0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8\\
    \cline{5-11}
    && && &\multicolumn{7}{c|}{Synthesized Program Cost}\\
    \hline
    phone-long-repeat & phone-1-long-repeat & 400 & 0.3& T & 80 & 94 & 80 & 67 & 54
    & 40 & 27\\
    phone-long-repeat & phone-2-long-repeat & 400 & 0.3&T & 80 & 94 & 80 & 67 & 54
    & 40 & 27\\
    phone-long-repeat & phone-5-long-repeat & 400 & 0.2& F &
    \\
    phone-long-repeat & phone-6-long-repeat \\
    phone-long-repeat & phone-7-long-repeat \\


    \hline
\end{tabular}
\end{center}
    \caption{Program Synthesized with dataset constructed from two benchmarks.}
    \label{table:mix}
\end{figure*}

